FleXR: A System Enabling Flexibly Distributed Extended Reality

Extended reality (XR) applications require computationally demanding functionalities with low end-to-end latency and high throughput. To enable XR on commodity devices, a number of distributed systems solutions enable offloading of XR workloads on remote servers. However, they make a priori decisions regarding the offloaded functionalities based on assumptions about operating factors, and their benefits are restricted to specific deployment contexts. To realize the benefits of offloading in various distributed environments, we present a distributed stream processing system, FleXR, which is specialized for real-time and interactive workloads and enables flexible distributions of XR functionalities. In building FleXR, we identified and resolved several issues of presenting XR functionalities as distributed pipelines. FleXR provides a framework for flexible distribution of XR pipelines while streamlining development and deployment phases. We evaluate FleXR with three XR use cases in four different distribution scenarios. In the results, the best-case distribution scenario shows up to 50% less end-to-end latency and 3.9x pipeline throughput compared to alternatives.

==> Makefile <==
filename=sample-authordraft

all: pdf

pdf:
	pdflatex-dev ${filename}
	- bibtex ${filename}
	pdflatex-dev ${filename}
	pdflatex-dev ${filename}
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' ${filename}.log) \
	  do pdflatex-dev ${filename}; done

clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi



==> sections/limitation_futurework.tex <==
%------------------------------------------------------------------------------
\section{Limitations and Future Work}
\label{sec:limfut}
%------------------------------------------------------------------------------

Even with its benefits, the current version of \sys\ has limitations, and there is future work.
Firstly, we did not explore the effects of different kernel granularities and that tradeoff space.
With the fine-grained kernels, the more parallelism can be achieved, but the benefit of parallelism can be compromised by the resource contentions.
Another limitation is that the current \sys\ does not have a feature to automatically determine how to distribute the entire workload by the environmental parameters such as client device capacity, network state, and the load on the remote server.
Some previous work leveraged linear solvers and resource profilers to make the offloading decisions with the static analysis~\cite{cuervo2010maui, chun2011clonecloud}.
In \sys, it is more complex because the parallel exeution of kernels causes resource contentions and additional overheads can be caused for distributing XR pipelines as described in \S~\ref{sec:evalresanaly}.
So, we put these limitations for future work.


